i-Algebra: Towards Interactive Interpretability of Deep Neural Networks

Providing explanations for deep neural networks (DNNs) is essential for their use in domains wherein the interpretability of decisions is a critical prerequisite. Despite the plethora of work on interpreting DNNs, most existing solutions offer interpretability in an ad hoc, one-shot, and static manner, without accounting for the perception, understanding, or response of end-users, resulting in their poor usability in practice. In this paper, we argue that DNN interpretability should be implemented as the interactions between users and models. We present i-Algebra, a first-of-its-kind interactive framework for interpreting DNNs. At its core is a library of atomic, composable operators, which explain model behaviors at varying input granularity, during different inference stages, and from distinct interpretation perspectives. Leveraging a declarative query language, users are enabled to build various analysis tools (e.g., "drill-down", "comparative", "what-if" analysis) via flexibly composing such operators. We prototype i-Algebra and conduct user studies in a set of representative analysis tasks, including inspecting adversarial inputs, resolving model inconsistency, and cleansing contaminated data, all demonstrating its promising usability.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section, we discuss some important issues related to interpretation and future work of \system.

\subsection{Integration of Diverse Interpretation Demands}

The empirical evaluations on our \system, which presents fidelity on solving a set of research use cases, indicate that \system can effectively incorporate a suite of toolchains to meet various user demands on interpreting DNNs.



\subsection{Scalability of \system}

As shown in Figure \ref{fig:stack}, our \system is built on a library of atomic operators including \emph{Identity}, \emph{Projection}, \emph{Selection}, \emph{Join} and \emph{Anti$-$Join}. Potentially, \system can be generalized to more scalable interpretation tasks beyond the multiple empirical cases above, which is supported by two reasons: (i) the operators library can be extended to involve more interpretation operators as an increasing number of interpretation works will be published; (ii) the flexible compositions of different operators can further extend the versatility of \system.
